Towards Robust Alignment of Language Models: Distributionally Robustifying Direct Preference Optimization

This study addresses the challenge of noise in training datasets for Direct Preference Optimization (DPO), a method for aligning Large Language Models (LLMs) with human preferences. We categorize noise into pointwise noise, which includes low-quality data points, and pairwise noise, which encompasses erroneous data pair associations that affect preference rankings. Utilizing Distributionally Robust Optimization (DRO), we enhance DPO's resilience to these types of noise. Our theoretical insights reveal that DPO inherently embeds DRO principles, conferring robustness to pointwise noise, with the regularization coefficient $\beta$ playing a critical role in its noise resistance. Extending this framework, we introduce Distributionally Robustifying DPO (Dr. DPO), which integrates pairwise robustness by optimizing against worst-case pairwise scenarios. The novel hyperparameter $\beta'$ in Dr. DPO allows for fine-tuned control over data pair reliability, providing a strategic balance between exploration and exploitation in noisy training environments. Empirical evaluations demonstrate that Dr. DPO substantially improves the quality of generated text and response accuracy in preference datasets, showcasing enhanced performance in both noisy and noise-free settings. The code is available at https://github.com/junkangwu/Dr_DPO.

==> chapters/7_conclusion.tex <==
\section{Conclusion}
In this study, we analyze DPO's robustness from a DRO perspective, highlighting its resilience to pointwise noise. We establish a link between DPO's regularization and DRO's robustness, showing that a smaller regularization parameter $\beta$ enhances stability against uncertain data. Our experiments confirm the crucial role of $\beta$ in noise resistance but uncover DPO's weakness against pairwise noise. To address this, we introduce a novel Distributionally Robustifying  DPO (Dr. DPO) framework with an additional parameter $\beta^{\prime}$ that balances data pair importance in training to enhance model robustness. 
The Dr. DPO's fine-tuning of exploration and exploitation could markedly improve the alignment of language models, assuring reliable performance in the presence of real-world noise.

% Our experimental validation is conducted on DPO and may not directly generalize to other models with different architectures or pre-training objectives. Further studies are needed to confirm the efficacy of Dr. DPO across a broader range of LLMs.

% \newpage
% \clearpage
% \section*{Impact Statements}
% This paper presents work whose goal is to advance the field of Machine Learning. There are many potential societal consequences of our work, none which we feel must be specifically highlighted here.
